Joint Prompt Optimization of Stacked LLMs using Variational Inference

Large language models (LLMs) can be seen as atomic units of computation mapping sequences to a distribution over sequences. Thus, they can be seen as stochastic language layers in a language network, where the learnable parameters are the natural language prompts at each layer. By stacking two such layers and feeding the output of one layer to the next, we obtain a Deep Language Network (DLN). We first show how to effectively perform prompt optimization for a 1-Layer language network (DLN-1). Then, we present an extension that applies to 2-layer DLNs (DLN-2), where two prompts must be learned. The key idea is to consider the output of the first layer as a latent variable, which requires inference, and prompts to be learned as the parameters of the generative distribution. We first test the effectiveness of DLN-1 in multiple reasoning and natural language understanding tasks. Then, we show that DLN-2 can reach higher performance than a single layer, showing promise that we might reach comparable performance to GPT-4, even when each LLM in the network is smaller and less powerful.

==> experiments.tex <==
\section{Experiments and Results}
\label{sec:exp}

We design and conduct a set of experiments to help answer two main research questions: \textbf{Q1:} Can we outperform APE and In-Context Learning (ICL) with a DLN-1? \textbf{Q2:} Does network depth provide further improvement upon DLN-1?

\subsection{Experimental Setup}
\label{sec:exp:exp_setup}

\paragraph{Datasets and Tasks}

We adopt a set of eight NLP and reasoning tasks commonly used in prior work studying zero- or few-shot learning capabilities of LLMs \cite{lu2022fantastically,gao2021making,srivastava2022beyond,suzgun2022challenging,bansal2020learning}. We focus on classification tasks.  For tasks adopted from BigBench-Hard (BBH)~\cite{suzgun2022challenging} (\hyper, \nav~and \logic\footnote{We only use the variant with seven objects.}), we use the 250 data points provided by BBH as test set. 
We take the remaining data points from BigBench~\cite{srivastava2022beyond} that were not included in BBH, and randomly split them (evenly) into training and validation sets. 
For tasks adopted from \cite{lu2022fantastically} (\mpqa, \trec, and \subj), we randomly sample 400 and 250 data points from their training and test sets, respectively. We use the original validation sets.
For tasks adopted from Leopard~\cite{bansal2020learning} (\disaster~and \airline), we randomly sample 400, 250, and 250 data points as training, valid, and test. 
We list all tasks and their statistics in Table~\ref{tab:data_stats} in the Appendix.

We use accuracy as the evaluation metric. 
Specifically, given an input, we compare a system's output string against the ground-truth output string provided by the dataset.
We score 1 if the two strings are identical and 0 otherwise. 
Before the comparison, we process the strings from both the model output and the ground-truth to deal with issues like tokenization and capitalization. 
In all our DLN experiments, we perform a hyperparameter search and run the same hyperparameter setting with three random seeds. 
We report the test accuracy averaged over three seeds corresponding to the hyperparameter setting that achieves the highest average validation accuracy.
We report details of the hyperparameter search in the App.~\ref{app:implementation}.  

Throughout this paper, we use OpenAI's \gptthree model, specifically \dvthree, as the backbone to our proposed systems unless otherwise specified. 

\paragraph{Baseline Systems}
We compare the DLN against two classes of baseline systems. 
First, we test a set of systems equipped with the same backbone (i.e., \dvthree):
\begin{itemize}[leftmargin=10pt]
    \item \texttt{0-shot}: Given an input, the LLM is required to generate the answer in a zero-shot manner. 
    \item \texttt{CoT} \cite{wei2022chain}: Given an input, the LLM is first queried to generate a reasoning path with the prompt \cmd{``Let's think step by step''}. Then, conditioned on the input and its first output, the LLM is queried to generate an answer. This is the zero-shot version of CoT.
    \item \texttt{ICL}: Given an input as well as five data points as in-context examples, the LLM is queried to generate an answer. The five examples are randomly sampled from the training set. 
    \item \texttt{KATE} \cite{liu2021makes}: Given an input, we retrieve the five most similar data points from the training set using an off-the-shelf sentence encoder, and use them as in-context examples.
    \item \texttt{APE} \cite{zhou2022large}: The LLM is queried to generate a pool of candidate prompts for the task given few input-output pair examples. The candidate prompts are evaluated on a validation set to find the best performing instruction prompt. The best instruction is then used for 0-shot evaluation. We optimize the prompt over both 15 and 400 examples (\texttt{APE-15} and \texttt{APE-400} respectively).
\end{itemize}
Additionally, we compare against one of the most advanced LLMs to date, \gptfour. 
We test \texttt{0-shot} and \texttt{ICL} settings with \gptfour. 

\subsection{DLN-1}
\label{sec:1L-results}
Our first set of experiments evaluates the 1-layer language network (DLN-1) described in Sec.~\ref{sec:prompt_optimization}. Table~\ref{tab:one-layer} presents results on the full suite of test tasks. We see that it matches the performance of the best \dvthree-based method on the \nav, \disaster, and \airline tasks and narrowly beats the best \dvthree baseline on \logic and \mpqa.
On \hyper, \trec, and \subj, DLN-1 significantly outperforms the best \dvthree baseline (by about 20, 10, and 7 percentage points, respectively).
On \hyper, \trec, and \disaster, it even surpasses \gptfour baselines (pink highlighting)---unsurprisingly underperforming \gptfour on all other tasks.
DLN-1's excellent performance on \hyper, a BigBench-Hard~\cite{suzgun2022challenging} task about ordering adjectives according to linguistic convention, is a surprise. To better understand it, we show the final prompt in Fig.~\ref{fig:hyper_prompt}. We see that the prompt contains both instructions and a list of examples from the training set. These examples were automatically chosen by the optimizer based on their impact on the performance. This can be seen as a combination of KATE, which selects training examples to put in context based on their similarity with the test example, and APE, which selects the prompt based on its performance.

\begin{table}[t!]
\scriptsize
    \centering
    \caption{Test accuracy averaged over three random seeds of a shallow, 1-layer language network (DLN-1) compared to baselines both on \dvthree and \gptfour. For trainable systems (i.e., APE and DLN-1), we report the 95\% confidence interval. \dvthree{} is \sethlcolor{lightblue}\hl{blue} and \gptfour is \sethlcolor{lightpink}\hl{pink}.}
    \begin{tabular}{l||llll|lll|ll}
        \toprule
          & \multicolumn{4}{c}{\textbf{BigBench Hard}} & \multicolumn{3}{|c}{\textbf{NLU}} & \multicolumn{2}{|c}{\textbf{Leopard}}\\
          \midrule
          & \hyper & \nav & \dateund & \logic & \mpqa & \trec & \subj & \disaster & \airline  \\
        \midrule
        \rowcolor{lightblue}
        \texttt{0-shot} &            60.8 & 64.1 & 56.4 & 45.9 & 88.0 & 61.9 & 61.7 & 81.6 & 75.6 \\
        \rowcolor{lightblue}
        \texttt{CoT} &        65.7 & 61.9 & 71.5 & 41.1 & 55.6 & 51.9 & 59.3 & 54.4 & 41.5 \\
        \rowcolor{lightblue}
        \texttt{ICL} &        55.6 & 56.5 & 62.1 & 36.7 & 87.2 & 80.0 & 76.4 & 81.2 & 82.7 \\
        \rowcolor{lightblue}
        \texttt{KATE} &       71.1 & 56.9 & 61.1 & 44.4 & 88.4 & 77.6 & 71.1 & 76.0 & 81.6  \\
        \rowcolor{lightblue}
        \texttt{APE-15} &               68.5{\tiny$\pm$5.5} & 67.3{\tiny$\pm$7.7} & 32.1{\tiny$\pm$28.6} & 45.5{\tiny$\pm$4.7} & 85.5{\tiny$\pm$4.6} & 71.3{\tiny$\pm$5.5} & 61.3{\tiny$\pm$7.2} & 54.8{\tiny$\pm$14.6} & 83.5{\tiny$\pm$3.5}  \\
        \rowcolor{lightblue}
        \texttt{APE-400} &               65.5{\tiny$\pm$4.7} & 56.9{\tiny$\pm$32.9} & 23.5{\tiny$\pm$14.1} & 45.6{\tiny$\pm$12.4} & 84.9{\tiny$\pm$9.7} & 72.0{\tiny$\pm$1.7} & 63.7{\tiny$\pm$9.2} & 60.3{\tiny$\pm$37.4} & 82.3{\tiny$\pm$10.0}  \\
        \midrule
        \rowcolor{lightblue}
        \texttt{DLN-1} & 91.9{\tiny$\pm$3.0} & 67.1{\tiny$\pm$7.6} & 55.7{\tiny$\pm$4.5} & 47.5{\tiny$\pm$2.1} & 88.5{\tiny$\pm$2.5} & 89.7{\tiny$\pm$3.2} & 83.2{\tiny$\pm$6.5} & 81.7{\tiny$\pm$6.5} & 83.2{\tiny$\pm$5.5}  \\
        \midrule
        \rowcolor{lightpink}
        \texttt{0-shot} & 65.1 & 72.0 & 78.2 & 67.2 & 78.3 & 73.2 & 65.8 & 76.3 & 86.4  \\
        \rowcolor{lightpink}
        \texttt{ICL} & 85.4 & 76.6 & 78.2 & 69.0 & 88.9 & 79.5 & 92.4 & 77.4 & 88.5  \\
        \midrule
        \rowcolor{lightpink}
        \texttt{DLN-1} & 95.2 & 77.1 & 74.3 & 69.1 & 91.1 & 89.5 & 93.1 & 82.1 & 85.9  \\
        \bottomrule
    \end{tabular}
    \label{tab:one-layer}
\end{table}

\begin{figure}
\begin{tcolorbox}[fonttitle=\small\fon{pbk}\bfseries,
fontupper=\scriptsize\sffamily,
enhanced,
left=2pt, right=2pt, top=2pt, bottom=2pt,
title=DLN-1 prompt on Hyperbaton]
When constructing a sentence with multiple adjectives, the order should be opinion, size, age, shape, color, origin, material, and purpose. Adjectives of the same type should be listed in descending order from largest to smallest. When adjectives of different types are used, the order should be opinion, size, age, shape, color, origin, material, and purpose. For example, in the phrase ``massive ancient chair'' size (massive) should come before age (ancient). Examples: little old-fashioned Russian silver rectangular ship; silly large old leather hiking chair; brand-new spherical Mexican sweater; enormous old spherical green Nigerian exercise car; medium-size triangular wool eating ship; good square brown Egyptian ship; lovely massive drinking monkey; archaic circular white plastic shoe. In each of the following examples, the adjective order is wrong. Identify the correct adjective order:
\end{tcolorbox}
\caption{\label{fig:hyper_prompt}The final prompt of the DLN-1 on Hyperbaton includes not only instructions but also examples from the training set. These samples were automatically chosen by the prompt optimization. In a way, this approach combines in-context learning and prompt optimization.
}
\end{figure}

\subsection{DLN-2}
\label{exp:two-layer}
Next we investigate the effectiveness of depth through experiments with 2-layer language networks (DLN-2) on tasks where we expect depth to be most useful, and on which DLN-1 significantly underperforms the \gptfour 0-shot baseline, i.e., \nav, \dateund, and \logic~\cite{suzgun2022challenging}. 

Since the \nav, \dateund and \logic~\cite{suzgun2022challenging}) tasks from BigBench-Hard require more complex spatial and temporal reasoning, they are the ones where we most expect a decomposition into subtasks to be helpful.
We use these datasets for a more extensive comparison against DLN-2 in Table~\ref{tab:two-layer}. We also include \subj as an example where DLN-1 performs well (even outperforming the \gptfour 0-shot baseline), since we are interested to see to what extent DLN-2 can further push performance.

Our DLN-2 is trained end-to-end. We describe in Appendix~\ref{app:exp_detail} a layerwise training procedure and its results but we found it to work consistently worse than end-to-end training.

\sethlcolor{lightblue}
As shown in Table~\ref{tab:two-layer} (highlighted in \hl{blue}), DLN-2 provides a boost to DLN-1 on average.
On \nav, DLN-2 successfully outperforms the \gptfour 0-shot baseline and \gptfour ICL by 5\% accuracy points.
On \dateund, DLN-2 further improves the performance of DLN-1, outperforming all single layer networks, but is far from matching \gptfour, even in 0-shot.
On \logic, DLN-2 fails to match the performance of DLN-1 and significantly trails \gptfour performance. This could point to a deficiency of the approximate posterior distribution or to the fact that we need a deeper network; we leave this for future work.
On \subj, DLN-2 achieves further improvement even though DLN-1 already greatly outperforms the \gptfour 0-shot baseline. DLN-2 provides a more than 20\% absolute improvement over 0-shot \gptfour.

\begin{table}[t!]
\small
\centering
\caption{DLN-2 test accuracy averaged over three random seeds. We highlight settings using \dvthree and \gptfour backbones \sethlcolor{lightblue}\hl{blue} and \sethlcolor{lightpink}\hl{pink}, respectively.}
    \begin{tabular}{ll||cccc||c}
        \toprule
        && \nav & \dateund & \logic & \subj & \textbf{Avg. Acc.}  \\
        \midrule
        \rowcolor{lightblue}
        & \texttt{0-shot} & 64.1 & 56.4 & 45.9 & 61.7 & 57.0  \\
        \rowcolor{lightblue}
        & \texttt{APE} & 67.3 & 32.1 & 45.5 & 71.1 & 54.0 \\
        \rowcolor{lightblue}
        & \texttt{DLN-1} & 67.1 & 55.7 & 47.5 & 83.2 & 63.4 \\
        \rowcolor{lightblue}
        \multirow{-4}{*}{\dvthree} & \texttt{DLN-2} & 82.9 & 63.9 & 45.2 & 85.9 & 69.5 \\
        \midrule
        \rowcolor{lightpink}
        & \texttt
{0-shot} & 72.0 & 78.2 & 67.2 & 65.8 & 70.8 \\
        \rowcolor{lightpink}
        \multirow{-2}{*}{\gptfour} & \texttt{ICL} & 76.6 & 78.2 & 69.0 & 92.4 & 79.1 \\
        \midrule
        \bottomrule
    \end{tabular}
    \label{tab:two-layer}
\end{table}

==> related.tex <==
\section{Related Work}
\paragraph{Prompt-Based Machine Learning}
GPT-3~\cite{brown2020language} demonstrated that sufficiently trained, sufficiently large language models are few-shot learners.
This launched a new paradigm in NLP called in-context learning (ICL), or simply prompting. Research and tinkering have now extended it beyond traditional NLP tasks~\cite{liu2023pre}.
\citet{liu2023pre} provide an excellent survey of how prompting has developed in the last several years---a development that DLNs rely on and extend.

Despite the success of prompting, challenges remain.
For instance, small changes to a prompt can have significant downstream impacts~\cite{min-etal-2022-rethinking}---which has given rise to the packed field of prompt engineering~\cite{liu2023pre}.
\citet{liu2021makes} likewise showed that LLM performance can depend heavily on the choice of examples included in the prompt as in-context demonstrations: constructing the prompt with samples that are semantically similar to the test example helps significantly.
This approach has since been key to several works~\cite{rubin2021learning, su2022selective, lazaridou2022internet}.

The discovery of chain-of-thought prompts (CoT) marked a major advance in prompting:
LLM performance improves markedly when the prompt includes examples of intermediate reasoning steps~\cite{wei2022chain} (few-shot CoT), or simply instructs the model to ``think step by step''~\cite{kojima2022large} (zero-shot CoT).
Like CoT, DLNs break a problem down into intermediate steps; however, they operationalize these steps as separate LLM calls, each defined by its own learned prompt.
Since the introduction of CoT, prompting techniques have evolved to be more dynamic and iterative.
Recent methods often operate recursively, with the prompt to an LLM containing LLM-generated text from a previous model call.

RECITE~\cite{sun2022recitation} is a CoT-based method that decomposes question-answering into two steps: reciting the relevant knowledge stored in model parameters, then generating the answer. In Self-ask~\cite{press2022measuring}, a model is prompted to ask and answer follow-up questions before answering an input question. \citet{creswell2022selection} decompose the question-answering problem into two interleaved steps: selecting supporting evidence from an LLM and then inferring an answer from an LLM that uses that evidence. Similarly, \citet{zhou2022least} decompose questions into a sequence of sub-questions then answer each of them in turn, via sequential calls to an LLM, and \citet{khot2023decomposed} induce an LLM to generate a basic `control flow' that calls distinct LLM modules. \citet{yoran-etal-2023-answering} generate multiple independent chains of reasoning for a question, then process them using a meta-reasoner and predict the answer. And ReAct~\cite{yao2022react} generates reasoning traces and task-specific actions from LLMs operating in an interleaved manner. It achieves strong performance on multi-hop question answering and interactive decision making benchmarks.
      
A related class of methods uses  `self-talk,' where an LLM is prompted to ingest, evaluate, then possibly act on its own previous output. It is a precursor to DLNs, although without our layer-based conceptual framework nor our learning formulation. Self-critique~\cite{saunders2022self}, prompts LLMs to find flaws in previous LLM generations, then integrate the critique as feedback and refine the generation accordingly. \citet{shinn2023reflexion} propose Reflexion, which pairs ReAct~\cite{yao2022react} with this kind of self-reflection/critique and a memory module to help an agent improve its performance over several trials. \citet{kim2023language} propose a prompting scheme whereby an agent recursively criticizes and improves its output to solve computer tasks. In Self-refine~\cite{madaan2023selfrefine}, an LLM generates an output, then the same model is prompted to provide multi-aspect feedback on its output; finally, the model refines its previous output given its feedback. For improved planning in robotic control scenarios, \citet{huang2022inner} enable LLMs to conduct an inner monologue that leverages environment feedback and other inputs. \citet{hao2023reasoning} propose Reasoning as Planning, which repurposes an LLM as both a world model and a reasoning agent. Their method incorporates a planning algorithm based on Monte Carlo Tree Search to effectively explore the reasoning space. Coincident with our work, \citet{du2023improving} present a ``society of minds'' approach, whereby multiple language model instances propose and debate individual reasoning processes iteratively to arrive at a final answer. And simultaneously, \citet{yao2023tree} propose Tree of Thoughts (ToT), an extension of CoT that enables LLMs to make more deliberate decisions through self-evaluation, look ahead, and backtracking over multiple proposed reasoning paths. Generally, these methods do not use an explicit optimization procedure as DLNs do. On the other hand, \citet{welleck2022generating} propose a Self-Correct method that adds a trainable, possibly smaller corrector module on top of a base LLM---and explains that multiple correctors can be stacked. Distinct from DLNs, the corrector is trained by gradient descent on its parameters, to which the authors assume full access.


\paragraph{Augmented LLMs}
A related set of work focuses on prompting LLMs to use external tools---e.g., by generating code for API calls and conditioning on the returned text. These methods also tend to use repeated calls to a model with a growing or dynamic prompt that incorporates API returns. Consider MindsEye~\cite{liu2022mind}, which enables physical reasoning in LLMs by calling the MuJoCo engine to simulate scenarios described in text, then translating the simulation results back into text for a prompt. Another example of augmentation adds the ability to query search engines, as in Self-ask~\cite{press2022measuring}. And most recently, \citet{cai2023large} proposed a method by which LLMs can construct their own tools, implemented as Python utility functions, for a given task. That method operates somewhat like 1-layer prompt optimization in DLNs, but with a different output. \citet{mialon2023augmented} provides a thorough survey of tool-augmented LLMs.

\paragraph{Prompt Optimization} Techniques based on notions of self-talk and self-evaluation align naturally with automatic prompt optimization---a core function in DLNs. Early work in this category includes Autoprompt~\cite{shin2020autoprompt}, which performs a gradient-based search for `trigger' tokens, which coax a masked language model to perform some task like sentiment classification; and GRIPS~\cite{prasad2022grips}, which splits instruction prompts into phrases, then uses a set of phrase-level operations (e.g., delete, swap, paraphrase, add) to optimize the instruction. \citet{deng2022rlprompt} argue that `enumeration-then-selection' heuristics for optimizing discrete prompts do not explore the prompt space systematically. They take an RL approach to overcome this problem, training a policy network, via soft Q-learning with a suitably designed and stabilized reward function, to generate effective prompts. In-context policy iteration~\cite{brooks2022incontext} offers another RL-based approach to prompt learning. The method iteratively updates the contents of a prompt---which defines the policy of an LLM-based agent---through trial-and-error interaction with an environment. Most relevant to DLNs,~\citet{zhou2022large} present Automatic prompt engineer (APE). APE optimizes an initial prompt by searching over a pool of candidates to maximize a score function. APE demonstrates that an LLM can be used both to generate prompt candidates and to score them---i.e., according to the log probability of a groundtruth output under the LLM given the prompt candidate. We use an APE-inspired approach in DLNs and we cast the proposal/scoring functions as elements of variational inference. In~\cite{xu2023wizardlm}, an initial set of instructions is rewritten automatically, step by step, into more complex instructions. This recalls prompt optimization across layers in DLNs, but the goal in~\cite{xu2023wizardlm} is to generate improved instruction data for fine-tuning a single LLM. Finally, we note an alternative to finding human readable prompts: optimizing continuous prompts~\cite{liu2023pre}, a.k.a. soft prompts. These are out of scope for us, since we assume no access to LLM internals.


\paragraph{Multi-Layer LLM systems}
Several recent works compose LLMs as nodes in a computational graph, which is the core idea of DLNs. Some work cited above can be seen as instances of this idea. For example, selection-inference~\cite{creswell2022selection} operates like a graph in which selection LLM nodes feed into inference LLM nodes to compose a single reasoning step, and multiple reasoning steps can be chained together. Similarly, \citet{khot2023decomposed} induce an LLM to generate a basic ``control flow'' that calls distinct LLM modules. \citet{wu2022ai} propose AI chains, an interactive system of chained LLMs based on a set of ``LLM primitive'' operations. They conduct a 20-person user study in which participants modify chains, and find this process to improve task performance, transparency, and controllability. Although our work on DLNs is also limited to linear networks (i.e., chains), we learn to modify their component operations. \citet{dohan2022language} unify LLMs and graphical models as ``language model cascades''. Specifically, they cast LLM compositions as graphical models with string-valued random variables.\footnote{Earlier work by \citet{miao2016language} also treated strings as random variables.} They show how scratchpad \cite{nye2021show}, chain-of-thought \cite{wei2022chain}, tool use~\cite{mialon2023augmented}, and several other prompting strategies fit their formalism. DLNs can likewise be considered an instance of language model cascade, because of that framework's generality. However, going beyond the conceptual work of~\citet{dohan2022language}, we present an effective technique for doing inference in an LLM-based graphical model and we apply learned networks of LLMs to several downstream tasks.


==> symbols.tex <==
\def\pih{{\pi_{t + \nicefrac{1}{2}}}}
\def\pitt{{\pi_{t+1}}}
\def\bpi{{\boldsymbol{\pi}}}
\newcommand{\pit}{{\pi_{t}}}
\newcommand{\tpitt}{\tilde{\pi}_{t+1}}

\def\piopt{{\pi^\ast}}
\newcommand{\grad}[1]{\nabla J(#1)}
\newcommand{\hgt}[1]{\hat g_t{(\pit)}}

\newcommand{\gradphi}[1]{\nabla \phi(#1)}
\newcommand{\breg}[2]{D_{\phi}(#1, #2)}



\newcommand{\inner}[2]{\langle #1,\, #2 \rangle}
\newcommand{\normsq}[1]{\left\|#1 \right\|_{2}^{2}}
\newcommand{\norm}[1]{\left\|#1 \right\|}
\newcommand{\indnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\indnormsq}[2]{\left\|#1\right\|_{#2}^{2}}
\newcommand{\dnormsq}[1]{\left\|#1\right\|_{*}^{2}}



\def\zh{{z_{t + \nicefrac{1}{2}}}}
\def\ah{{a_{t + \nicefrac{1}{2}}}}

\newcommand{\F}{{\Pi}}
\newcommand{\f}{{\pi}}
\newcommand{\ft}{{\pi_{t}}}
\newcommand{\ftt}{{\pi_{t+1}}}
\newcommand{\fth}{{\pi_{t + \nicefrac{1}{2}}}}


\newcommand{\pidist}{{p^\pi}}
\newcommand{\pitdist}{{p^{\pi_{t}}}}
\newcommand{\pittdist}{{p^{\pi_{t+1}}}}
\newcommand{\pipdist}{{p^{\pi'}}}

\newcommand{\lse}{{\textrm{logsumexp}}}


\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}
\newcommand{\transpose}{^\mathsf{\scriptscriptstyle T}}
\def\eps{{\epsilon}}


\newcommand{\gradt}{\nabla J(\pit)}
\newcommand{\tgradt}{\hat{g}(\pit)}

\newcommand{\etat}{{\eta_t}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\cA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\cF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\cH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\cP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\cS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sE{{\mathbb{E}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\def\II{{\mathcal{I}}}
\def\PP{{\mathcal{P}}}
\newcommand{\TT}{\mathcal{T}}


\newcommand{\OP}{\textsc{Op-}}
\newcommand{\RF}{\textsc{Reinforce~}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\Lphi}{L_{\phi}}


\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\def\FMAPG/{{FMA-PG}}
\def\DFMAPG/{{DFMA-PG}}
\def\SFMAPG/{{SFMA-PG}}


\newcommand{\tht}{{\theta_{t}}}
\newcommand{\thtt}{{\theta_{t+1}}}
\newcommand{\gradf}[1]{\nabla f(#1)}
\newcommand{\sgradf}[1]{\nabla \tilde{f}(#1)}


\newcommand{\mpqa}{\texttt{Mpqa}\xspace}
\newcommand{\trec}{\texttt{Trec}\xspace}
\newcommand{\subj}{\texttt{Subj}\xspace}
\newcommand{\disaster}{\texttt{Disaster}\xspace}
\newcommand{\airline}{\texttt{Airline}\xspace}
\newcommand{\hyper}{\texttt{Hyper.}\xspace}
\newcommand{\nav}{\texttt{Nav.}\xspace}
\newcommand{\dateund}{\texttt{Date.}\xspace}
\newcommand{\logic}{\texttt{Logic.7}\xspace}

\definecolor{darkgreen}{HTML}{005e19}
\definecolor{lightblue}{HTML}{edf6ff}
\definecolor{lightpink}{HTML}{ffeded}
\definecolor{lightgreen}{HTML}{f2ffed}
\definecolor{lightyellow}{HTML}{fcfaca}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\cmd}[1]{\textcolor{darkgreen}{\textbf{\code{#1}}}}
\newcommand{\dlnone}{\texttt{DLN-1}\xspace}
\newcommand{\dlntwo}{\texttt{DLN-2}\xspace}
\newcommand{\dvthree}{\texttt{DaVinci-003}\xspace}
\newcommand{\dvtwo}{\code{text-davinci-002}\xspace}
\newcommand{\gptfour}{\code{GPT-4}\xspace}
\newcommand{\gptthree}{\code{GPT-3}\xspace}
\newcommand{\curie}{\code{curie}\xspace}

\lstdefinelanguage{yaml}{
  keywords={true,false,null,y,n,h,input, next\_prompt, prompt, prompt_memory, message, backward_infos, backward_info, loss, template, message_alternatives},
  keywordstyle=\color{darkgray}\bfseries,
  ndkeywords={for, if, in, endfor, endif, END},
  ndkeywordstyle=\color{delim}\bfseries,
  identifierstyle=\color{black},
  sensitive=false,
  breaklines=true,
  columns=fullflexible,
  basewidth = {.6em},
  breakindent = {0em},
  tabsize=1,
  aboveskip=0em,
  belowskip=0em,
  %moredelim=[l]{}{:},
  %comment=[l]{\#},
  morecomment=[s]{/*}{*/},
  commentstyle=\color{purple}\ttfamily,
  stringstyle=\color{blue}\ttfamily,
  %morestring=[l]{-}{},
  morestring=[b]',
  morestring=[b]",
  alsoletter={.},
  morekeywords={backward_info.input, backward_info.output, backward_info.loss, backward_info.target}
}
